Cross Copy Network for Dialogue Generation

In the past few years, audiences from different fields witness the achievements of sequence-to-sequence models (e.g., LSTM+attention, Pointer Generator Networks, and Transformer) to enhance dialogue content generation. While content fluency and accuracy often serve as the major indicators for model training, dialogue logics, carrying critical information for some particular domains, are often ignored. Take customer service and court debate dialogue as examples, compatible logics can be observed across different dialogue instances, and this information can provide vital evidence for utterance generation. In this paper, we propose a novel network architecture - Cross Copy Networks(CCN) to explore the current dialog context and similar dialogue instances' logical structure simultaneously. Experiments with two tasks, court debate and customer service content generation, proved that the proposed algorithm is superior to existing state-of-art content generation models.

==> 2_Background.tex <==
% \section{Background}

% In this section, We will introduce our baseline model: Sequence-to-sequence attention model, Pointer Generation Networks, Transformer.
% These three models are closely related to our model.


% \subsection{Sequence-to-sequence attentional model}
% Recently, there has been a surge of work proposing to build the Natural Language Generation within a seq2seq+attention\cite{bahdanau2014neural} framework. 
% It has great potential for various tasks in natural language, such as machine translation, text summaries, etc.
% The model usually uses RNN (contain RNN, LSTM) structure and has an encoder and a decoder.
% The role of the encoder maps the context to a vector, and the task of the decoder is to convert this vector into the text to be generated.
% We get the encoder hidden state $h_i$ of the contenxt through the encoder, in the each time step $t$, Decoder received representation of original context information produce decoder state $s_t$. 

% \begin{equation}
% V_t = v^Ttanh(W_h*h_i+W_s*s_t+b_h)
% \end{equation}
% As shown in the formula, $v$, $W_h$, $W_s$, $b_h$ represents the parameters to be learned during training. 

% With attention mechanism, we calculated as:
% \begin{equation}
% a^t = softmax(V_t)
% \end{equation}
% We can get attention distribution $a_i$, it represent a probability distribution of source words. Then, we can get context vector $h_t$:
% \begin{equation}
% h^c_t = \sum(a_i^t*h_i)
% \end{equation}
% We will concatenated context vector $h^c_t$ and decoder hidden state $s_t$ through linear transformation get vocabulary distribution $P_v$:
% \begin{equation}
% P_v = softmax(W^v(W^p*[h^c_t, s_t]+b_p)+b^v)
% \end{equation}

% Therefore, $W^v$, $b_v$, $W^p$ and $b_p$ represents the parameters to be learned during training. 
% According to vocabulary probability distribution $P_v$,  we get final distribution preict words $w$:
% \begin{equation}
% P(w) = P_v(w)
% \end{equation}


% \subsection{Pointer Generation Networks}
% Unlike the sequence-to-sequence+attention model, the Pointer Generation Networks uses the attention mechanism as a pointer to select token in the context, and then obtains an expanded vocabulary distribution beyond the original vocabulary distribution.
% We have got encoder hidden state $h_i$, decoder state $s_t$, decoder input $x_t$, context vector $h_t^c$ and attention distribution $a^t$ in section 3.1.
% First, we need to calculate the generation probability $p_gen$ at each time step $t$:
% \begin{equation}
% p_{gen} = \sigma(W_h^**h^c_t+W_s^**s_t+W_x^**x_t+b)
% \end{equation}
% The $W_h^*$, $W_s^*$ and $W_x^*$ are parameters which need training.
% The $\sigma$ is sigmod function.


% In Pointer Generation Networks, wo through attention distribution and vocabluary distribution get expanded vocabulary $P_e$.
% In the decode, the output sequence's probability distribution from expanded vocabluary $P_e$:
% \begin{equation}
% P_e = p_{gen}P_v(w)+(1-p_{gen})\sum_{i:w_i=w}a^t_i
% \end{equation}
% As shown above, $w$ is Out-Of-Ovcabulary (OOV) word.
% In the trainging, model will be selected to copy the word from context by attention distribution $a^t$. if the word will be generated not in context, the $p_{gen}$ is zero. 


% \subsection{Transformer}
% Transformer\cite{vaswani2017attention} is a new network architecture which based solely on attention mechanisms.
% In order to deal with the problem that RNN cannot be parallelized, there have been some solutions using CNN, such as Google's ByteNet\cite{kalchbrenner2016neural}, Facebook proposed FairSeq\cite{gehring2017convolutional}, etc.
% This model proposed a particular attention named "Scaled Dot-Product Attention", it's input consists of queries $Q$ and keys $K$ of dimension $d_k$, and values $V$ of dimension $d_v$.
% This is a self attention mechanism, it can be as a set of key-value pairs to an output.
% The $Q$, $K$ and $V$ are matrices of learning parameters.
% Self attention can be computed as:
% \begin{equation}
% Attention(Q, K, V) = softmax(\frac{Q*K^T}{\sqrt{d_k}})V
% \end{equation}
% The self-attention mechanism can connect information at different positions on the input sequence, and then calculate a certain expression of the entire sequence.


% And the reason for dividing by $d_k$ is that when the dimension $d_k$ of the key is particularly large, the dot product may become very large, causing the subsequent softmax function to enter a small gradient range, which is not conducive to training.


% Therefore, in each word embedding dimension, we execute a multi-block attention mechanism in parallel and then concatenated and once again projected, which is called Multi-Head Attention.
% \begin{equation}
% Multi-Head(Q, K, V) = Concat(head_1,...,head_h)W^O
% \end{equation}
% \begin{equation}
% head_i = Attention(QW_i^Q, KW_i^K, VW_i^V) 
% \end{equation}
% The $W^O$, $W_i^Q$, $W_i^K$ and $W_i^V$  are learnable parameters. 


% Because the transformer does not use any recurrence or convolution structure, in order for the model to use the sequence information of the input sequence, some information that can express the absolute or relative position of each part of the input sequence must be introduced. 
% The method adopted by the transformer is positional encoding.
% Before entering the encoder and decoder, the input is encoded. 
% The vector dimension after encoding is dmodeldmodel. 
% Specifically, encoding using sine and cosine functions:
% \begin{equation}
% PE(pos,2i) = sin(pos/10000^{{2i}/d_model})
% \end{equation}
% \begin{equation}
% PE(pos,2i+1) = cos(pos/10000^{{2i}/d_model})
% \end{equation}
% The $pos$ is position and $i$ is the dimension.


% We compare the advantages and disadvantages of self-attention, recurrence structure, and convolutional structure from three aspects. 
% The first is the computational complexity of each layer, the second is the amount of computation that can be performed in parallel, and the last is the length of the path that the network depends on for a long time.
% The comparison shows that self-attention performs best.


%  Using transformers to be able to handle longer dependencies, without recurrence structure and convolutional structure, making model training faster.

==> 2_Problem_formulation.tex <==
% \section{Model}

% \begin{figure*}
%     \centering
%     \includegraphics[width=1\textwidth]{encoder.png}
%     \caption{The encoder of the network structure that we proposed \textbf{CCN}. It is divided into three levels: (1) \textbf{Utterance layer}: used to merge and encode role information and word level information; (2) \textbf{Dialogue layer}: used to encode sentence level information; (3) \textbf{Transformer layer}: use the multi-heads attention to extract the subspace after encoding the dialogue information, each head is equivalent to a separate channel, and can be used to independently extract different effective features}
%     \label{fig:encoder}
% \end{figure*}

% In this section, we introduce the proposed model, the Cross Copy Network. 
% The model has three major components:

% \begin{enumerate}
% \item \textbf{Target Cases Representation}: we obtain two attention distributions at the utterance layer and the dialogue layer, then merge the two distributions to obtain our final attention distribution (see Sec. 2.2);
% \item \textbf{Similar Cases Representation}: we use a pre-trained language model to obtain a vector representation of the dialogue, thereby obtaining similar cases (see Sec. 2.3);
% \item \textbf{Cross Copy}: we learn two pointers distributions, used to achieve internal (vertical) copy and external (horizontal) copy (see Sec. 2.4).
% \end{enumerate}

% \subsection{Problem formulation}
% Given a dialogue $\mathbf{D}=\{(\mathbf{U}, \mathbf{R})^L\}$ containing $L$ utterances, the $\mathbf{U}$ and $\mathbf{R}$ stand for utterance and role of speaker, respectively, where each utterances in the dialogue is expressed as $\mathbf{U_i}=\{w_{i1}, w_{i2},...,w_{il}\}$, and the $l$ represents the length of the utterances. To distinguish \textbf{SC} and original context. We define the original context (historical dialogue) as \textbf{Target Case}. 


% In order to help readers better understand the model, the definitions of the important notations are illustrated as follows:
% \begin{itemize}
% \setlength{\itemsep}{0pt}
% \setlength{\parsep}{0pt}
% \setlength{\parskip}{0pt}
%     \item $\mathbf{D}$: dialogue in the legal context or customer service context;
%     \item $\mathbf{U}$: the utterance in $\mathbf{D}$;
%     \item $\mathbf{R_i}$: the role of the speaker of $\mathbf{U_i}$;
%     \item $\mathbf{S_{ij}}$: concatenating the role information with each word of utterance, so, $\mathbf{S_{ij}}=[\mathbf{R_i},w_{ij}]$;

% \end{itemize}
% Note that $\mathbf{U}$, $\mathbf{R}$ and $\mathbf{S}$  represent the embedding representations of the corresponding variables in the list.
